Attacking Byzantine Robust Aggregation in High Dimensions

Training modern neural networks or models typically requires averaging over a sample of high-dimensional vectors. Poisoning attacks can skew or bias the average vectors used to train the model, forcing the model to learn specific patterns or avoid learning anything useful. Byzantine robust aggregation is a principled algorithmic defense against such biasing. Robust aggregators can bound the maximum bias in computing centrality statistics, such as mean, even when some fraction of inputs are arbitrarily corrupted. Designing such aggregators is challenging when dealing with high dimensions. However, the first polynomial-time algorithms with strong theoretical bounds on the bias have recently been proposed. Their bounds are independent of the number of dimensions, promising a conceptual limit on the power of poisoning attacks in their ongoing arms race against defenses. In this paper, we show a new attack called HIDRA on practical realization of strong defenses which subverts their claim of dimension-independent bias. HIDRA highlights a novel computational bottleneck that has not been a concern of prior information-theoretic analysis. Our experimental evaluation shows that our attacks almost completely destroy the model performance, whereas existing attacks with the same goal fail to have much effect. Our findings leave the arms race between poisoning attacks and provable defenses wide open.

==> chapters/existing.tex <==
\section{Why do Existing Approaches Fail?}
\label{sec:existing}

Table \ref{tab:robust_gaurantees} summarizes prior approaches. Several techniques provide better robustness that arithmetic mean computation, such as median~\cite{robuststats-book}, trimmed mean~\cite{yin2021byzantinerobust}, krum~\cite{krum}, and others. These approaches have bounds that are proportional to $d$, the number of dimensions. Attacks against them can induce significant bias in practice. Since $d$ can grow large in modern neural networks, one desires that bias is independent of $d$. 

Techniques such Filtering, No-Regret, DnC, and others assure the bias remains unaffected by $d$~\cite{zhu2023byzantinerobust, shejwalkar2021manipulating,diakonikolas2019sever}. 
%
These state-of-the-art algorithms all employ the same underlying principle and blueprint as proposed in ~\cite{diakonikolas2018robust}, which is captured as a meta-procedure in Algorithm~\ref{alg:existing_algos}. The procedure checks the spectral norm of the covariance of the given sample $Y$. If it falls below a constant threshold, they return the arithmetic mean of gradients. However, when the spectral norm exceeds the threshold, they activate their unique outlier removal subroutines, which may involve eliminating gradients or adjusting their weights until the spectral norm falls below the threshold. 

Our observation is that the above procedures will achieve their ideal behaviour, i.e., bias independent of $d$, provided that the gradient distributions are nearly isotropic. One can view the threshold they use as corresponding to the maximum variance of uncorrupted gradient distributions across all directions. Attempting to bias the mean requires aligning corrupted gradients in some specific direction, to avoid them cancelling each other, which increases the variance in that direction and the overall spectral norm. Hence the check for spectral norm is used, or equivalently, checks on the maximum eigenvalue (variance) can be used.
%
But, the above principle is only true when the distribution is nearly isotropic---the variance in all directions is nearly equal and close to a maximum value.

Are gradient distributions in practice nearly isotropic? This is often not the case. Fig~\ref{fig:non_isotropic} shows the variance of (uncorrupted) gradients along different eigenvectors of the covariance matrix, as seen when training on the popular MNIST dataset. The gradient distribution is {\em not} approximately isotropic. The variance along different eigenvector directions varies significantly---it is about $10^{-38}$ for about $90\%$ of the directions and $10^{-6}$ for the one with maximum variance. Fig~\ref{fig:non_isotropic} is representative of a broader empirical observation: There are many directions in the vector space where the benign variance is much smaller than the maximum. 

When the above phenomena occurs, any procedure based on the blueprint of Algorithm~\ref{alg:existing_algos} fails to guarantee that the bias is independent of $d$. A concrete attack strategy is as follows: Perform eigenvalue decomposition of the covariance matrix of benign gradients and order eigenvectors by increasing variance. Then, project the given gradients along each eigenvector. Now, shift an $\epsilon$ fraction of gradients along each eigenvector starting from the smallest. The shift is to 
any one side of the mean by a constant, chosen such that we limit the variance of the final shifted gradients to remain below the maximum variance. Note that for the covariance matrix, eigenvectors are orthogonal since the covariance matrix is a symmetric matrix. Orthogonal eigenvectors ensure shifts along one eigenvector will not affect the others. After repeating this process for all eigenvectors, except a few towards the end (which have large variance), we can project the gradients back to original basis to obtain our final corrupted gradients. The corrupted gradients will have a substantial bias of $O(\sqrt{\epsilon }\cdot s)$ along each eigenvector where $s^2$ is difference between maximum variance and benign variance along that eigenvector. The bias scales with $d$
because there are $d$ eigenvectors\footnote{When do we expect d eigenvectors? It happens in practice}, and along each (except for a last few) we corrupted by a constant. The spectral norm will be below the threshold, by construction, hence the check on Line 2 in Algorithm~\ref{alg:existing_algos} will return the simple arithmetic mean of the corrupted samples $Y$. Its L2 norm will be $O(\sqrt{\epsilon \cdot d})$, violating the desired guarantee. Appendix A details the attack procedure and its analysis. 

% Specifically, the adversary can replace $\epsilon$

% gradients in practice significantly deviates from these assumptions and is {\em not} approximately isotropic. We contend that we can exploit this aberration to craft potent attacks against these algorithms. Algorithms following these outlines will excel if the gradient distribution is isotropic.  This initiates outlier removal, which leverages the gradient distribution along the direction of maximum variance to eliminate outliers. Through multiple iterations, it clears outlier gradients in directions where the variance exceeds the threshold. In contrast, when dealing with a non-isotropic gradient distribution in practical setups, biasing the mean in a specific direction does {\em not} necessarily increase the spectral norm. In this context, an adversary can shift the mean in a direction to the extent that its variance along that specific direction increases, reaching a point just slightly lower than the maximum variance. An adaptive adversary can, therefore, manipulate the mean in all directions except the direction of maximum variance. This manipulation can result in a bias that scales with the number of dimensions. 



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{non_isotropic.png}
    \caption{This illustration showcases the variance of gradients for the initial layer of a ConvNet trained on MNIST along various eigenvectors of its covariance matrix.}
    \label{fig:non_isotropic}
\end{figure}



% \subsection{Security Property}
% The fundamental idea behind corrupting gradient vectors is straightforward: to introduce a substantial bias into the aggregated gradients, you need to position your corruptions far from the mean without arousing suspicion. This task becomes increasingly feasible as the number of parameters, or the dimension of gradient vectors, increases. In high-dimensional spaces, adversaries can place their corruptions in numerous directions. There are two fundamental approaches to consider when addressing this problem. From the defender's perspective, you can either choose to examine all directions for outliers or identify the directions that are most susceptible to containing corrupt data points. Both of these ideas raise several questions, such as whether it is efficient to check for outliers in all directions or if there exists a prioritized order in which directions are more likely to contain corrupt data points. Even if there is a precedence order, it prompts the question of whether it is adequate to inspect a fixed number of directions from the top of that order. Our assertion is that any approach adhering to the latter strategy is unlikely to succeed in a practical setting, such as gradient descent, where the distribution of data points varies significantly along each direction. We also claim that it is efficient to simultaneously check for outliers in all directions. You can refer to a detailed discussion addressing the aforementioned and other problems in Section ~\ref{sec:previouswork}.

% In this context, it is crucial to delve into what it precisely means to check for outliers and the criteria that form the basis for suspecting the presence of outliers along a specific direction. Building on the concept introduced regarding corruption at the beginning, it becomes evident that a direction where all data points closely align with the mean is less likely to contain corruption compared to a direction where data points are widely dispersed around their mean. Variance is the statistical measure that quantifies the same concept, which becomes readily apparent through Chebyshev's concentration inequality, applicable to any random variable $X$, $\mathbf{Pr}(|X - \mathbb{E}(X)| \geq a) \leq \frac{\text{Var}(X)}{a^2}$. This relationship implies that higher variance along a direction corresponds to an increased likelihood of points deviating significantly from its mean in that direction. This offers a compelling rationale for assessing the variance of gradient vectors in different directions and underscores the essential insight that if an adversary corrupts a point with the intention of inducing a significant shift in the mean along a specific direction, it will inevitably result in an increase in the variance along that direction. It is important to note that this increased variance can still be lower than the maximum variance of the uniform distribution over the benign gradients across all directions. 

% In the role of a defender, it's crucial to concentrate on directions with significantly higher variance compared to what would occur in the absence of corruption. This implies that the direction in which this difference is the greatest represents the direction along which the mean deviates the most due to corruption. However, we cannot solely focus on that particular direction, as the variance differences in other directions may not be as large but could still be significant enough to affect the mean. Therefore, if a defender chooses to assess variance in only a fixed number of directions, it would provide an advantage to the adversary, allowing corruption in more than the selected number of directions. We demonstrate that evaluating variance in all directions incurs a comparable computational cost to assessing it in a fixed number of directions on the order of $d$. Therefore, we opt to evaluate the variance of gradients in all directions. This distinguishes us from prior research in two significant ways. Firstly, we establish that the directions with substantial differences in variance (between the corrupted and benign cases) are the most vulnerable to corruption, as opposed to directions with high variances. Secondly, we opt to evaluate this difference in variance across all directions. Thus, we are the pioneers in introducing this as a security property called {\em panaromic robustness}. This property asserts that only when a set of $\epsilon$-corrupted points exhibit an arbitrarily small difference in variance compared to the expected variance in the benign case across all directions, can its empirical mean be considered a statistically optimal estimate of the benign mean.



==> chapters/final_attack.tex <==
%-------------------------------------------------------------------------------
\section{Final Attack}
\label{sec:final_attack}
%----------------------------------------------------------------------------

As previously established, BGRA is closely tied to high-dimensional robust mean estimation. Numerous federated learning protocols have been introduced ~\cite{zhu2023byzantinerobust, diakonikolas2019sever, shejwalkar2021manipulating}, leveraging the recently proposed optimal robust mean aggregators ~\cite{diakonikolas2018robust, gao2019robust, zhu2020robust}. Do these optimal robust mean aggregators efficiently scale for direct deployment in practical setups like federated learning where the dimensional can easily be in the order of $10^5$? 
No, these optimal robust mean aggregators primarily rely on assessing the spectral norm of input samples, which imposes a computational limitation on the number of dimensions they can effectively consider within a reasonable timeframe.
As proposed in ~\cite{zhu2023byzantinerobust}, the most natural approach to circumvent this computational limitation is to partition the gradients into intervals of a specified value (e.g., $1000$), and subsequently estimate the mean for each interval using the aforementioned robust mean aggregators. This approach leads to the development of state-of-the-art BGRA algorithms.  
An essential question to address is whether these algorithms maintain the worst-case guarantee provided by the underlying robust aggregator for high-dimensional gradients. 
We contend that this workaround does not provide optimal guarantees regarding the bias in the mean, potentially creating an opening for adversaries to devise attacks against it.
Therefore, we introduce a novel attack against the state-of-the-art BGRA algorithms, along with an analysis demonstrating how these algorithms can yield sub-optimal error guarantees, even when utilizing optimal robust aggregators.
\begin{algorithm}[t]
\caption{Attack against state-of-the-art algorithms for BGRA}
\label{alg:attack_algo}
\begin{algorithmic}[1] % Set the line numbering to start at 1
% \REQUIRE Input data
% \ENSURE Output data
\REQUIRE benign gradients $X = \{x_1, ..., x_n\}$, fraction of corruption $\epsilon$
\ENSURE $\epsilon$-corrupted gradients $Y = \{y_1, ..., y_n\}$ 
\STATE $\hat{\mu} = \frac{1}{n} \sum_{i=1}^n x_i$  \hspace{0.5cm} $\triangleright$ compute the mean of $X$
\STATE $\hat{\Sigma} = \frac{1}{n} \sum_{i=1}^n (x_i - \hat{\mu})(x_i - \hat{\mu})^{T}$
\hspace{0.5cm} $\triangleright$ Compute the sample covariance matrix of $X$
\STATE $w$, $v$ $\leftarrow$ eigenvalues and eigenvectors of $\hat{\Sigma}$
\STATE $v^{*}$ $\leftarrow$ sort $v$ in increasing the order of absolute values of $w$
\STATE $X' = \{x_1', ..., x_n'\}$ $\leftarrow$ project the input gradients along $v^*$ to get new components of each gradient in the rotated basis
\STATE $\hat{\sigma}_{max}^2$ $\leftarrow$ variance of last component of $X'$
\FOR{$i=0$ {\bfseries to} $i= n \cdot \epsilon - 1$}
    \STATE $\hat{\sigma_i}^2$ $\leftarrow$ variance of $i$-th component of each $x'$
    \STATE $|\mu'|_i = \sum_{j=0}^{n} |x_{j}'|_i$  \hspace{0.5cm} $\triangleright$ calculate benign mean of $i$-th component of $X'$.
    \STATE $s^2 = \hat{\sigma}_{max}^2 - \hat{\sigma_i}^2$ 
    \STATE $corr = n^{\frac{1}{2}} \cdot s$  \hspace{0.5cm} $\triangleright$ calculate the value for corruption 
    \IF {$|\mu'|_i \leq 0$}
        \STATE $|x'_i|_i = |\mu'|_i + corr$ \hspace{0.5cm} $\triangleright$ corrupt $i$-th component of $i$-th sample
    \ELSE
        \STATE $|x'_i|_i = |\mu'|_i - corr$
    \ENDIF
\ENDFOR

\STATE $Y = \{y_1, ..., y_n\}$ $\leftarrow$ project $X'$ back to original basis of input gradients 
\RETURN $Y$
\end{algorithmic}
\end{algorithm}
 The outline of our attack procedure is as follows: first, partition the gradient into fixed-size intervals, denoted as $c$, following the same approach employed by the considered BGRA algorithms. Next, utilize the Algorithm \ref{alg:attack_algo} to devise a corrupted set for each of these intervals. Finally, combine all the intervals to create a set of complete $\epsilon$-corrupted gradients of $d$ dimensions. All existing state-of-the-art BGRA algorithms solely evaluate the spectral norm of the covariance matrix of input gradients. In real gradient distributions, however, the variance along each direction can vary significantly, resulting in numerous eigenvectors of the covariance matrix having nearly negligible variance compared to the spectral norm. This observation forms the central insight behind our attack strategy ~\ref{alg:attack_algo}, where we aim to corrupt each fixed-size partition of gradients. 
Algorithm ~\ref{alg:attack_algo} operates based on the concept that if a corrupted data point is introduced into a benign data set along an eigenvector and increases the variance along that specific eigenvector to match the spectral norm's value, it ensures that the spectral norm of the entire set remains unaltered. This approach ultimately ensures that none of our introduced corruptions is filtered out by the current state-of-the-art BGRA algorithms, enabling us to establish a bias of $O(\sqrt{\epsilon})$ in each partition. This bias accumulates to $O(\sqrt{\epsilon \cdot d})$ in the mean of the entire gradient set. We demonstrate that adhering to Algorithm ~\ref{alg:attack_algo} yields a bias on the order of $O(\sqrt{\epsilon})$ for each gradient partition without impacting its spectral norm. Consider a set of benign gradients $X = {x_1, x_2, ..., x_n}$ where each $x_i$ is a $c$ dimensional vector, and without loss of generality, we will assess algorithm ~\ref{alg:attack_algo} on the first partition of the original gradients, i.e. first $c$ components.  \\

Let $\hat{\Sigma} \in \mathbb{R}^{c \times c}$ be the sample covariance matrix and $\hat{\mu} \in \mathbb{R}^c$ be the sample mean of the first partition of gradients, \\
$$ \hat{\Sigma} = \frac{1}{n} \cdot \sum_{i=1}^{n} (x_i - \hat{\mu})(x_i - \hat{\mu})^{T} $$ 
If we expand this covariance matrix in terms of the components of each $x_i$, this covariance matrix would be, where $z_i = x_i - \hat{\mu}$ and $|z_i|_j$ denotes $j$-th component of $z_i$
$$
\hat{\Sigma} = \frac{1}{n} \cdot
 \begin{pmatrix}
  \sum |z_i|_1^2 &  \sum |z_i|_1 |z_i|_2 & \cdots & \sum |z_i|_1|z_i|_c \\
  \sum |z_i|_2 |z_i|_1 & \sum |z_i|_2^2 & \cdots & \sum |z_i|_2|z_i|_c \\
  \vdots  & \vdots  & \ddots & \vdots  \\
  \sum |z_i|_c |z_i|_1 & \sum |z_i|_c |z_i|_2 & \cdots & \sum |z_i|_c^2 
 \end{pmatrix}
$$

To diagonalize this covariance matrix, we can project all $x_i$ along the eigenvectors of $\hat{\Sigma}$, sorting them in the order of increasing variance along each eigenvector. Let $X' = \{x_1', x_2', \cdots, x_n'\}$ be the projected set of gradients and , following the same notation, $z_i' = x_i' - \hat{\mu}'$, now the new covariance matrix would be, 

$$
\hat{\Sigma'} = \frac{1}{n} \cdot
 \begin{pmatrix}
  \sum |z_i'|_1^2 &  0 & \cdots &  0\\
  0 & \sum |z_i'|_2^2 & \cdots & 0 \\
  \vdots  & \vdots  & \ddots & \vdots  \\
  0 & 0 & \cdots & \sum |z_i'|_c^2 
 \end{pmatrix}
$$
where $\sum |z_i'|_1^2 \leq \sum |z_i'|_2^2 \dots \leq \sum |z_i'|_c^2$. We will shift a single point $x_1'$ along the first eigenvector having the minimum variance such that the variance along that direction equals the maximum variance, i.e. $\sum |z_i'|_c^2$. Assume the $k$ is the value of shift in $|x_1'|_1$ to increase the variance up to the maximum. As a result, $|\hat{\mu'}_{new}|_1 = |\hat{\mu'}|_1 + \frac{k}{n}$, this will change the covariance matrix as follows,  
{\footnotesize
\[
\hat{\Sigma'} = \frac{1}{n} \cdot
\begin{pmatrix}
\sum \left(|z_i'|_1 - \frac{k}{n}\right)^2 & \sum \left(|z_i'|_1 - \frac{k}{n}\right) |z_i'|_2 & \cdots & \sum \left(|z_i'|_1 - \frac{k}{n}\right) |z_i'|_c \\
\sum |z_i'|_2 \left(|z_i'|_1 - \frac{k}{n}\right) & \sum |z_i'|_2^2 & \cdots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
\sum |z_i'|_c \left(|z_i'|_1 - \frac{k}{n}\right) & 0 & \cdots & \sum |z_i'|_c^2
\end{pmatrix} 
\]

\[
+
\]

\[ \frac{1}{n} \cdot
\begin{pmatrix}

(|z'_1|_1 + k - \frac{k}{n})^2& \left(|z_1'|_1 + k - \frac{k}{n}\right) |z_1'|_2 & \cdots & \left(|z_1'|_1 + k - \frac{k}{n}\right) |z_1'|_c \\
|z_1'|_2 \left(|z_1'|_1 + k - \frac{k}{n}\right) & |z_1'|_2^2 & \cdots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
|z_1'|_c \left(|z_1'|_1 + k - \frac{k}{n}\right) & 0 & \cdots &  |z_1'|_c^2
\end{pmatrix} 
\]
}

On simplifying this expression, we will get a diagonal covariance with first and last entry as $\sum |z'_i|_c^2$. Eventually after shifting each of $n \cdot \epsilon$ gradients along one of the eigenvector with small variance, the final covariance matrix will have first $n \cdot \epsilon$ entries as $\sum |z'_i|_c^2$ (maximum variance). It shows that adding corruption using Algorithm \ref{alg:attack_algo} ensures that the covariance matrix of gradients remains diagonal and no entries becomes more than the maximum variance, hence it doesn't affect the spectral norm. As a result, all the state-of-the-art BGRA algorithm assessing spectral norm to filter out will not be able to remove the corruptions added through aforementioned strategy. This creates a bias of $O(1/n)$ in $n \cdot \epsilon$ directions which results in overall bias of $O(\sqrt{\epsilon})$ in the norm of mean of each partition of gradients. This bias in each partition of gradients adds up to $\frac{d}{c}$ times and results into a total bias of $O(\sqrt{\epsilon \cdot d})$ in the mean of complete gradients.

==> chapters/previous_attacks.tex <==
%-------------------------------------------------------------------------------
\section{Previous Attacks}
\label{sec:previous_attacks}
%-------------------------------------------------------------------------------

Even before the emergence of the current state-of-the-art BGRA algorithms, several robust aggregators such as trimmed mean, coordinate-wise median, krum, among others, were proposed for robust gradient aggregation. However, all these earlier aggregators offer sub-optimal error guarantees concerning mean bias, and numerous untargeted attacks exploiting these sub-optimal guarantees have been introduced. Although existing attacks do not perform effectively against the state-of-the-art BGRA algorithms, as demonstrated in ~\cite{zhu2023byzantinerobust}, it becomes evident in Section ~\ref{sec:final_attack} that these state-of-the-art BGRA algorithms ultimately yield more or less the same sub-optimal error guarantees when deployed for high-dimensional gradients because of their computational limitations. Our assertion is that previous attacks may not have been optimized sufficiently to evade the current state-of-the-art defenses, but it remains possible to devise potent attacks against these defenses as well. We will now examine certain earlier attack strategies and provide arguments as to why they are not particularly effective against a defender who evaluates the variance of input gradients.

\paragraph{Inner-Production Manipulation Attack (IMA)} 

\paragraph{Local Model Poisoning Attacks (for krum and median)}

==> chapters/solution.tex <==
%-------------------------------------------------------------------------------
\section{Our Approach and Challenges}
\label{sec:solution}
%-------------------------------------------------------------------------------

Until now, we've outlined the drawbacks of previous research, stressing that limiting the spectral norm of the gradient distribution isn't sufficient. Spectral norm confinement essentially restricts gradient variance to a uniform constant across all directions. Certainly, to simplify our approach, we will initially explore this issue in two dimensions. Subsequently, we will proceed to present a viable solution to the problem, which can be readily extended to higher dimensions. The fundamental concept behind bounding the gradient variance is to restrict the spatial distribution of gradients. For example, constraining only the spectral norm of the distribution, as done in previous works, is equivalent to placing a circular filter around the arithmetic mean of the corrupted gradients. Figure \ref{fig:benign_samples} vividly demonstrates this concept, displaying the distribution of benign gradients in a two-dimensional space, with significant variance observed in a specific direction. To control the gradients' structure, a defender can maintain gradients within a fixed threshold from the mean in all directions as depicted by the circular boundary. While this circular boundary effectively constrains movement in the horizontal direction, it provides adversaries with considerable freedom to maneuver in the vertical direction. As a result, a corrupted spatial distribution, as depicted in Figure \ref{fig:corrupted_samples}, can be accepted by this boundary, even though it differs significantly from the benign case in the vertical direction. Consequently, this allows for the successful manipulation of the mean along that direction. 
This highlights the optimal strategy: bounding the variance in each direction with varying thresholds. This allows the defender to utilize a non-symmetric boundary to regulate the gradient distribution effectively. Consequently, it eliminates any room for adversaries to manipulate the spatial distribution of gradients without pushing the corruptions outside the boundary. Is it feasible to establish such a precise boundary by evaluating variance in a fixed number of directions?

\begin{figure}
  \label{fig:circle_boundary}
  \centering
  \subfigure[Benign Samples]{
    \label{fig:benign_samples}
    \includegraphics[width=0.4\textwidth]{figs/circle_benign.jpg}
  }
  \subfigure[Corrupted Samples]{
    \label{fig:corrupted_samples}
    \includegraphics[width=0.4\textwidth]{figs/circle_corrupted.jpg}
  }
  \caption{Using a circular boundary to restrict the spatial distribution of gradients.}
\end{figure}

Since our approach differs significantly from previous works, we encounter novel challenges. We concentrate on tackling two primary challenges. The first involves devising a method to detect outliers in all directions, while the second pertains to the integration of our assessments across all directions to effectively eliminate the final outliers. To shed light on the challenges we face, let's delve further into the latter issue. We argue why prior approaches, which assess variance in a single predetermined direction or in a fixed number of directions (e.g., all eigenvectors of the covariance matrix of gradients, providing a reasonable representation of variance across all directions), fall short. When employing these prior approaches and projecting points along a specific direction, applying a threshold to label outliers, as proposed in ~\cite{diakonikolas2018robust}, offers a probabilistic guarantee that benign points won't be mistakenly removed. However, this situation worsens when repeating the process across multiple directions and removing the union of outliers from those directions. Even if we choose to employ a threshold-less brute-force approach, considering all possible combinations of $1 - \epsilon$ fraction of points to find the combination that approximates the variance as closely as the benign case in a specific direction, there's no guarantee that these $1 - \epsilon$ fraction of points will remain consistent across all directions. Moreover, attempting this in multiple directions becomes computationally expensive, and the situation deteriorates if the adversary deliberately avoids corrupting the directions the defender intends to examine.

As a defender, we will need access to two essential pieces of information: $\epsilon$ and an estimate of the covariance matrix ($\hat{\Sigma}$) of the uniform distribution over a set of benign gradients. Henceforth, when we mention the distribution of benign gradients, we are referring to the uniform distribution over the set of benign gradients for the sake of brevity. Our assertion is that this level of information is a necessary requirement to provide any statistically optimal guarantee in $d$ regarding the estimation of the benign mean in practical setups. We adopt an approach to depict {\em panaromic robustness} by means of a system of quadratic equations similar to ~\cite{kothari2017outlierrobust}. You can refer to the details and differences from ~\cite{kothari2017outlierrobust} in Section \ref{sec:ourapproach}. We are examining all conceivable combinations of $1 - \epsilon$ fraction of corrupted points, combined with an $\epsilon$ fraction of new points, to evaluate their variance. Our goal is to ensure that the variance of this new set of points closely approximates the variance of a uniform distribution over benign points in every direction ($\hat{\Sigma}$). 
We achieve the inclusion of all potential combinations by assigning binary weights to each point and incorporating them into our system of quadratic equations. Additionally, we have devised a concise set of quadratic equations that guarantees the variance of these weighted points closely approximates the variance corresponding to $\hat{\Sigma}$ in all directions. We employ a method rooted in semi-definite programming (SDP) relaxations and develop a degree-$2$ sum of squares algorithm ~\cite{kothari2017outlierrobust} to resolve our system of quadratic equations. Subsequently, we utilize the obtained solution to estimate the empirical mean of the set of benign gradients. We defer the detailed explanation of this in Section \ref{sec:ourapproach}.

We are the first to introduce a defense strategy that offers optimal guarantees within practical settings. Furthermore, we are the first to identify fundamental vulnerabilities that emerge in practical setups and effectively address them with our defense. Additionally, we successfully tackle the computational overhead and expand our analysis to encompass general distributions from ~\cite{kothari2017outlierrobust}, thereby providing an algorithm with guarantees tailored to our specific use case. This represents a significant advancement, not just in terms of enhancing the existing solutions, but also in providing the accurate foundational property that should underlie every defense strategy for addressing this problem.
